Endotrivial modules for cyclic $p$-groups and generalized quaternion groups via Galois descent

In this paper, we investigate the group of endotrivial modules for certain $p$-groups. Such groups were already been computed by Carlson-Th\'evenaz using the theory of support varieties; however, we provide novel homotopical proofs of their results for cyclic $p$-groups, the quaternion group of order 8, and for generalized quaternion groups using Galois descent and Picard spectral sequences, building on results of Mathew and Stojanoska. Our computations provide conceptual insights into the classical work of Carlson-Th\'evenaz.

==> galoisdescentold.tex <==
In this section, we prove that Galois descent holds for $\StMod(kG)$ for $G$ a cyclic $p$-group or a generalized quaternion group.  These are precisely the cases where $G$ is a $p$-group of $p$-rank 1, and so $G$ has a unique nontrivial elementary abelian subgroup~$H$.  

If $G \cong C_{p^{n}}$, then $H$ is the subgroup $C_p$, with quotient $G / H \cong C_{p^{n-1}}$. If $G \cong Q_{2^n}$ is a (generalized) quaternion group, $H \cong C_2$ is the center of $G$.  In the case $G \cong Q_8$, the quotient $G / H$ is isomorphic to the Klein four-group $(C_2)^2$. If $G \cong Q_{2^n}$ for $n \geq 4$, then the quotient is isomorphic to a dihedral group $G / H \cong D_{2^{n-1}}$. Note that in all cases, $H$ is normal (and central) in $G$.

Specifically, in the first section, we establish that we have Galois extensions
$$k^{tG} \to k^{tH}$$
for the $G$ and $H$ above, using a result of Rognes along with a base change argument.  In the following sections, we prove that these Galois extension are faithful, using a criterion of Rognes on the contractibility of Tate constructions. These are \cref{thm:ktCpfaithful} for $G$ a cyclic $p$-group, \cref{thm:ktq8faithful} for $G$ the quaternion group of order 8, and \cref{thm:ktq2nfaithful} for $G$ a generalised quaternion group. 

% We have used \cref{quillen} as the motivating theorem of this paper, but in the special cases we will interest ourselves in in this paper (cyclic groups and generalised quaternion groups), there is only a single elementary abelian $p$-subgroup, so that the `decomposition' in \cref{quillen} consists of a single object. In this special case, we may rephrase the decomposition through Rognes' theory of Galois descent. From this point of view, the decomposition can be proved throughly purely homotopical methods. We turn to this in this section. 

\section{Galois extensions of ring spectra}

We begin with some basic definitions.

Let $f \colon R \to S$ be a map of $\mathbb{E}_\infty$-ring spectra. We call it a \textbf{$G$-Galois extension} if there is a $G$-action on $S$ such that the natural maps $R \to S^{hG}$ and $S \otimes_R S \to F(G_+,S)$ are weak equivalences. We say that the Galois extension is \textbf{faithful} if $S$ is faithful as an $R$-module. That is, if $M$ is an $R$-module such that $S \otimes_R M$ is contractible, then so is $M$ itself.

Whenever we have a faithful Galois extension, we have a good theory of descent called \textbf{Galois descent}, which has been studied by Gepner-Lawson, Meier, and Mathew-Stojanoska, among others:

\begin{thm}[\cite{GepnerLawson2016-ps} \cite{ms}]
	If $f \colon R \to S$ is a faithful $G$-Galois extension of $\mathbb{E}_\infty$-rings, then we have a natural equivalence of $\infty$-categories
	\[\mi{Mod}(R) \simeq \mi{Mod}(S)^{hG}\,\text{.}\]
\end{thm}

As the Picard spectrum functor commutes with limits, we deduce that we have an equivalence of connective spectra:
\[\mf{pic}(R) \simeq \tau_{\geq0}(\mf{pic}(S)^{hG})
\]
Therefore, we can use the homotopy fixed point spectral sequence to compute $\Pic(R) \cong \pi_0\big(\pic(S)^{hG}\big)$. Our general strategy to computing $\Pic(R)$ is to construct a faithful Galois extension $R \to S$ such that we understand $\Mod(S)$ or $\pic(S)$ well.  Specifically, we prove that we have natural maps $k^{tG} \to k^{tH}$ that are Galois ectensions for all aforementioned $G$ and $H$.


%We now prove that we have a theory of Galois descent for $\StMod(kG)$ in the cases $G \cong C_{p^n}$ (Theorem \ref{thm:ktCp}), $G \cong Q_8$ (Theorem \ref{thm:ktq8}), and $G \cong Q_{2^n}$ (Theorem \ref{thm:ktq2n}).  That is, we will first show that for a certain subgroup $H$, we have Galois extensions $k^{hG} \to k^{hH}$ by a general argument of Rognes \cite{rognes}. We then show that these Galois extensions are faithful by evaluating the relevant Tate spectral sequences. By Theorem \ref{thm:basechange}, this implies that we have faithful Galois extensions $k^{tG} \to k^{tH}$.

\begin{rmk}
    It is worth mentioning that Dade's theorem on endotrivial modules of elementary abelian groups is also known to have a proof using the theory of Galois descent, or rather, reverse Galois descent; see \cite{Mathewtorus2015-yg}. Let $k$ be the field $\mathbb{F}_p$, and let $A$ be an elementary abelian $p$-group $(C_p)^n$. One can construct a fiber sequence of classifying spaces $$B\Z^n \to BA \to B^2\Z^n \simeq B\mathbb{T}^n$$
    where $\mathbb{T}^n$-denotes the $n$-torus. Mathew uses this to prove that there exist faithful $\mathbb{T}^n$-Galois extensions of ring spectra 
    \[k^{h\T^n} \to k^{hA} \qquad \text{and} \qquad k^{t\T^n} \to k^{tA}\]
    In this case, it is the source rather than the target which is understood well, and Mathew proves conditions for an element in the Picard group of $k^{t\mathbb{T}^n}$ to descend to the Picard group of $k^{tA}$.  This, along with a computation of $\Pic(k^{t\mathbb{T}^n})$, shows that $\Pic(k^{tA})$ is cyclic.
\end{rmk}

\section{Galois extensions for cochain algebras}

In this section, we prove that for $G$ a $p$-group of $p$-rank 1, with unique nontrivial elementary abelian subgroup~$H$, we have natural maps $k^{tG} \to k^{tH}$ that are $G/H$-Galois extensions. We first show that we have Galois extension $k^{hG} \to k^{hH}$ on homotopy fixed points, and then invoke a base change argument to deduce the desired result. Our main tool is the following result of Rognes.

\begin{thm}[{\cite[Prop. 5.6.3]{rognes}}]
    \label{rognesgalois}
    Let $\Gamma$ be a finite discrete group, and $P \to X$ a principal $\Gamma$-bundle.  Suppose that $X$ is path-connected and $\pi_1(X)$ acts nilpotently on $H_*(\Gamma;k)$. Then the map of cochain $k$-algebras $F(X_+,k) \to F(P_+,k)$ is a $\Gamma$-Galois extension.
\end{thm}

We sketch the idea of the proof. To see that $F(X_+,k) \simeq F(P_+,k)^{h\Gamma} $ follows from properties of principal $\Gamma$-bundles. Namely, we have that the (right) action of $\Gamma$ on $P$ induces a left $\Gamma$ action on $F(P_+,k)$, which is compatible with the identification $X \simeq P_{h\Gamma}$. That is, of $X$ as the homotopy orbits of the action of $\Gamma$ on $P$.

The interesting part is showing that $$F(P_+,k) \otimes_{F(X_+,k)} F(P_+,k) \simeq F\big(\Gamma_+, F(P_+,k)\big)$$ As a tensor product of ring spectra, the homotopy groups of the left-hand side may be computed using the K{\"u}nneth spectral sequence:
$$E^2_{s,t} \cong \Tor_{s,t}^{\pi_*(A)}(\pi_*(B), \pi_*(B)) \Rightarrow \pi_{s+t}(B \otimes_A B)$$

Meanwhile, the homotopy groups of the right hand side can be computed using the Eilenberg--Moore spectral sequence with $k$-coefficients via the identification $F\big(\Gamma_+, F(P_+,k)\big) \simeq F\big((\Gamma \times P)_+,k\big)$: 
$$E^2_{s,t} \cong \Tor_{s,t}^{H^*(X;k)}\big(H^*(P;k), H^*(P;k)\big) \Rightarrow H^{-(s+t)}(P \times_X P;k)$$

%this spectral sequence is derived by taking cohomology with $k$ valued coefficients of the cobar construction.

%Further note that $H^*\big((BH \times_{BG} BH)_+; k\big) \cong H^*\big((BG \times G/H)_+; k\big) \cong \pi_{-*}(F(G/H_+, k^{hH}))$.

Since $\pi_*(F(X_+,k)) \cong H^*(X;k)$, we see that the $E_2$-pages of these spectral sequences agree.  Moreover, the filtrations are identified as well, as both can be viewed as being derived from the cobar construction. Therefore, if both spectral sequences converge strongly, then we obtain an equivalence between their targets, which is what we desired. 

The K{\"u}nneth spectral sequence is always strongly convergent, and a theorem of Shipley \cite{shipleysseq} guarantees convergence of the Eilenberg--Moore spectral sequence if the hypotheses of Theorem \ref{rognesgalois} are satisfied ($\Gamma$ a finite discrete group, $X$ is path-connected and $\pi_1(X)$ acts nilpotently on $H_*(\Gamma;k)$). 

\begin{rmk}
Rognes proved \cref{rognesgalois} in more generality than is needed for this paper - the argument holds for stabily dualizable topological groups $G$, so long as certain finiteness conditions are imposed.  Namely, $\pi_0(G)$ is finite, and $H^*(X;k)$ and $H^*(P;k)$ are finite in each degree.
\end{rmk}

We apply \cref{rognesgalois} to the fibre sequence $G / H \to BH \to BG$, where $G$ is a cyclic $p$-group or a generalised quaternion group, and $H$ is its elementary abelian $p$-subgroup. Notice that $BG$ is path-connected, and $G$, as a $p$-group, acts nilpotently on $H_*(G/H;k)$. We deduce that we have a $G/H$-Galois extension $F(BG_+,k) \to F(BH_+,k)$. Now since $G$ acts trivially on~$k$, these function spectra are naturally identified with homotopy fixed points, so we have proved the following results:

\begin{thm}
	\label{thm:khCp}
	The natural ring map $k^{hC_{p^n}} \to k^{hC_p}$ is a $C_{p^{n-1}}$-Galois extension of $\mathbb{E}_\infty$-rings.
\end{thm}

\begin{thm}
\label{thm:khq}
	The natural ring map $k^{hQ_{2^n}} \to k^{hC_2}$ is a $Q_{2^n}/C_2$-Galois extension of $\mathbb{E}_\infty$-rings.
\end{thm}

\subsection{passage to tate constructions}

\todo: Say more to show that $(k^{tC_2})^{hQ/H} \simeq k^{tQ}$

From material that we discuss in the Appendix, namely \cref{thm:greenleestate}, this will yield Galois extensions $k^{tG} \to k^{tH}$ for all aforementioned $G$ and $H$.  Observe that if $G$ is $C_p$, $C_{p^n}$, or $Q_{2^n}$, then the rings $\pi_{-*}(k^{hG}) \cong H^*(G;k)$ are Cohen--Macaulay.  In fact, for these choice of $G$, $\pi_{-*}(k^{hG}) \cong H^*(G;k)$ is free over a polynomial subalgebra $A \cong k[x]$.  Moreover, we can identify these particular Tate constructions $k^{tG}$ as localization away from the ideal $(x)$.  This is in particular a finite localization, and hence we have pushout diagrams exhibiting base-change.

\begin{center}
    \begin{tikzcd}
k^{hC_{p^n}} \arrow[d] \arrow[r] & k^{hC_p} \arrow[d] \\
k^{tC_{p^n}} \arrow[r]           & k^{tC_p}          
\end{tikzcd}
\qquad
\begin{tikzcd}
k^{hQ_{2^n}} \arrow[d] \arrow[r] & k^{hC_2} \arrow[d] \\
k^{tQ_{2^n}} \arrow[r]           & k^{tC_2}          
\end{tikzcd}
\end{center}

The discussion above and the following result of Mathew provide a proof for \cref{thm:ktCp} and \cref{thm:ktq}. 
    
    \begin{lem}[{\cite[Prop. 3.7]{Mathewtorus2015-yg}}]
    \label{thm:basechange}
    (Faithful) $G$-Galois extensions are stable under base-change.  
\end{lem}

\begin{thm}
	\label{thm:ktCp}
	The natural ring map $k^{tC_{p^n}} \to k^{tC_p}$ is a $C_{p^{n-1}}$-Galois extension of $\mathbb{E}_\infty$-rings.
\end{thm}

\begin{thm}
\label{thm:ktq}
	The natural ring map $k^{tQ_{2^n}} \to k^{tC_2}$ is a $Q_{2^n}/C_2$-Galois extension of $\mathbb{E}_\infty$-rings.
\end{thm}




We remark that it suffices to show that $k^{hG} \to k^{hH}$ is a faithful $G/H$-Galois extension.  By the previous lemma, this implies that Galois descent holds for $k^{tC_{p^n}} \to k^{tC_p}$ and $k^{tQ_{2^n}} \to k^{tC_2}$.  However, the proof proceeds in exactly the same way (i.e. computing the Tate spectral sequence).  Furthermore, we require the HFPSS calculations involving  $k^{tC_{p^n}} \to k^{tC_p}$ and $k^{tQ_{2^n}} \to k^{tC_2}$ in our Picard spectral sequence calculations.  


\section{Faithful Galois extensions}

Our next goal is to prove that the Galois extensions $k^{tC_{p^n}} \to k^{tC_p}$ and $k^{tQ_{2^n}}\to k^{tC_n}$ are faithful.  We will repeatedly invoke the following criterion of Rognes that our Galois extensions are faithful.

\begin{thm}[{\cite[Prop. 6.3.3]{rognes}}]
\label{thm:rognesfaithful}
	A $G$-Galois extension $f \colon R \to S$ is faithful if and only if the Tate construction $S^{tG}$ is contractible.
\end{thm}

This is especially useful because of the existence of the multiplicative \textbf{Tate spectral sequence}: if~$X$ is a spectrum with a $G$-action for some group $G$, then there is a spectral sequence
\[E_2^{st} = \widehat{H}^s\big(G; \pi_t(X)\big) \Rightarrow \pi_{t-s}(X^{tG})\,\text{,}\]
with differentials $d_r\colon E_r^{s,t} \to E_r^{s+r,t+r-1}$, which lets us compute the homotopy groups of $X^{tG}$ in terms of more readily accessible Tate cohomology groups. Moreover, we can leverage naturality and the cofibre sequence $X_{hG} \to X^{hG} \to X^{tG}$ to compare and import many differentials between the homotopy orbit spectral sequence, the homotopy fixed point spectral sequence, and the Tate spectral sequence. Notably though, in the (generalised) quaternion case, we will find an additional nontrivial $d_4$-differential which does not come from a HFPSS.

%We will draw all of our spectral sequences in the Adams grading $(t-s,s)$, which is a transformation of the standard grading coming from the $E_2^{s,t}$-page of the HFPSS and Tate spectral sequence.  This allows one to easily read off the homotopy groups $\pi_{t-s}$ of the abutment, and typically makes the spectral sequence figures more compact.

\section{For Cyclic $p$-groups}


\begin{thm}
	\label{thm:ktCpfaithful}
	The $C_{p^{n-1}}$-Galois extension $k^{tC_{p^n}} \to k^{tC_p}$ of $\mathbb{E}_\infty$-rings is faithful.
\end{thm}

\begin{proof}
    Our goal is to compute the Tate spectral sequence 
	\[ E_2^{st} \cong \wh{H}^{s}\big(C_{p^{n-1}};\pi_t k^{hC_p}\big) \Ra \pi_{t - s} (k^{hC_p})^{tC_{p^{n-1}}}\]
	and show that the Tate spectrum $(k^{tC_p})^{tC_{p^{n-1}}}$ is contractible. To do so, we recall that the natural map from homotopy fixed points to Tate fixed points allows us to import differentials from the HFPSS
	\[E_2^{st} = H^s\big(C_{p^{n-1}};\pi_t k^{hC_p}\big) \Ra \pi_{t - s}(k^{hC_{p}})^{hC_{p^{n-1}}}\,\text{.}\]
	In fact, this spectral sequence identifies with the Hochschild--Serre spectral sequence associated to the (central) extension $C_p \to C_{p^{n}} \to C_{p^{n-1}}$, which is well-understood. We review this spectral sequence, distinguishing between the cases where $p = 2$ and $p$ is odd.
	
	If $p = 2$, then the $E_2$-page, which has been illustrated in \cref{E2lhsC2}, is of the form
	\[E_2 \cong H^*(C_{2^{n-1}};k) \otimes H^*(C_2;k) \cong k[x] \otimes k[e]\,\text{,}\]
	where $e$ is of $t$-degree $-1$ because of the degree switch $\pi_{-t}(k^{hC_2}) \cong H^{t}(C_2;k)$. 
	\begin{figure}
        \centering
        \begin{sseqpage}[
        Adams grading,
        yscale =0.8,
        xscale =0.8,
        x tick step = 2, 
        x range = {-6}{2},
        y range = {0}{5},
        x label = {$t - s$},
        y label = {$s$},
        grid = chess, 
        classes = { minimum width = 0.2cm, minimum height = 0.2cm },
        run off = .-.]
        \class(0, 0)
        \class["e" {right, xshift = -0.2cm}](-1, 0)
        \class["x" {right, xshift = -0.2cm}](-1, 1)
        \class(-2, 0)
        \class(-2, 1)
        \class(-2, 2)
        \class(-3, 0)
        \class(-3, 1)
        \class(-3, 2)
        \class(-3, 3)
        \class(-4, 0)
        \class(-4, 1)
        \class(-4, 2)
        \class(-4, 3)
        \class(-4, 4)
        \class(-5, 0)
        \class(-5, 1)
        \class(-5, 2)
        \class(-5, 3)
        \class(-5, 4)
        \class(-5, 5)
        \class(-6, 0)
        \class(-6, 1)
        \class(-6, 2)
        \class(-6, 3)
        \class(-6, 4)
        \class(-6, 5)
        \d2(-1, 0)
        \d2(-3, 0)
        \d2(-5, 0)
        \d2(-2, 1)
        \d2(-4, 1)
        \class(-7, 3)
        \d2(-6, 1)
        \d2(-3, 2)
        \d2(-5, 2)
        \d2(-4, 3)
        \class(-7, 5)
        \d2(-6, 3)
        \class(-6, 6)
        \d2(-5, 4)
        \class(-7, 7)
        \d2(-6, 5)
        \end{sseqpage}
            \caption{The Adams-graded $E_2$-page of the HFPSS computing $\pi_*(k^{hC_{2^n}})$.  The circles denote a $k$-summand. All components are isomorphic to $k$ as a $k$-vector space. We have explicitly indicated the multiplicative generators. The nonzero differentials have been illustrated.}
        \label{E2lhsC2}
    \end{figure}
    An argument involving e.g. transgression proves that $d_2(e) = x^2$, while $d_2(x) = 0$ for degree reasons. By multiplicativity, this determines the remaining differentials. The $E_3$-page has been illustrated in \cref{E3lhsC2}, and the spectral sequence collapses.
    \begin{figure}
        \centering
        \begin{sseqpage}[
        Adams grading,
        yscale =0.8,
        xscale =0.8,
        x tick step = 2, 
        x range = {-6}{2},
        y range = {0}{3},
        x label = {$t - s$},
        y label = {$s$},
        grid = chess, 
        classes = { minimum width = 0.2cm, minimum height = 0.2cm },
        run off = .-.]
        \class(0, 0)
        \class(-1, 1)
        \class(-2, 0)
        \class(-3, 1)
        \class(-4, 0)
        \class(-5, 1)
        \class(-6, 0)
        \end{sseqpage}
            \caption{$E_3=E_\infty$-page of the Hochschild--Serre spectral sequence associated to the extension $C_2 \to C_{2^n} \to C_{2^{n-1}}$. There are no remaining differentials, and the spectral sequence collapses.}
        \label{E3lhsC2}
        \end{figure}
    
    We can now again compute $\pi_{t - s} (k^{tC_{2^n}})$ via the HFPSS.  Recall that the $E_2$ page (Figure \ref{fig:E2ktCpn}) is given by
    \[E_2^{s,t} \cong H^{-s}\big(C_{2^{n-1}}; \pi_t(k^{tC_2})\big) \cong k[x] \otimes k[t^{\pm1}]\,\text{.}\]
    
    \begin{figure}
    \centering
    \begin{sseqpage}[
    Adams grading,
    yscale =0.8,
    xscale =0.8,
    x tick step = 2, 
    x range = {-3}{5},
    y range = {0}{4},
    x label = {$t - s$},
    y label = {$s$},
    grid = chess, 
    classes = { minimum width = 0.2cm, minimum height = 0.2cm },
    run off = .-.]
    
    \class(-3, 0)
    \class(-3, 1)
    \class(-3, 2)
    \class(-3, 3)
    \class(-3, 4)
    \class(-3, 5)
    \class(-3, 6)
    \class(-2, 0)
    \class(-2, 1)
    \class(-2, 2)
    \class(-2, 3)
    \class(-2, 4)
    \class(-2, 5)
    \class(-2, 6)
    \class(-1, 0)
    \class(-1, 1)
    \class(-1, 2)
    \class(-1, 3)
    \class(-1, 4)
    \class(-1, 5)
    \class(-1, 6)
    \class(0, 0)
    \class(0, 1)
    \class(0, 2)
    \class(0, 3)
    \class(0, 4)
    \class(0, 5)
    \class(0, 6)
    \class(1, 0)
    \class(1, 1)
    \class(1, 2)
    \class(1, 3)
    \class(1, 4)
    \class(1, 5)
    \class(1, 6)
    \class(2, 0)
    \class(2, 1)
    \class(2, 2)
    \class(2, 3)
    \class(2, 4)
    \class(2, 5)
    \class(2, 6)
    \class(3, 0)
    \class(3, 1)
    \class(3, 2)
    \class(3, 3)
    \class(3, 4)
    \class(3, 5)
    \class(3, 6)
    \class(4, 0)
    \class(4, 1)
    \class(4, 2)
    \class(4, 3)
    \class(4, 4)
    \class(4, 5)
    \class(4, 6)
    \class(5, 0)
    \class(5, 1)
    \class(5, 2)
    \class(5, 3)
    \class(5, 4)
    \class(5, 5)
    \class(5, 6)
    \d2(-1, 0)
    \d2(-2, 1)
    \d2(1, 0)
    \d2(0, 1)
    \d2(-1, 2)
    \d2(-2, 3)
    \d2(3, 0)
    \d2(2, 1)
    \d2(1, 2)
    \d2(0, 3)
    \d2(-1, 4)
    \d2(5, 0)
    \d2(4, 1)
    \d2(3, 2)
    \d2(2, 3)
    \d2(1, 4)
    \d2(5, 2)
    \d2(4, 3)
    \d2(3, 4)
    \d2(5, 4)
    \class(-3, 7)
    \class(-1, 7)
    \class(1, 7)
    \class(3, 7)
    \d2(-2, 5)
    \d2(0, 5)
    \d2(2, 5)
    \d2(4, 5)
    \class(6, 1)
    \class(6, 3)
    \class(6, 5)
    \class(5, 7)
    \d2(6, 1)
    \d2(6, 3)
    \d2(6, 5)
    \class(-4, 2)
    \class(-4, 4)
    \class(-4, 6)
    \d2(-3, 0)
    \d2(-3, 2)
    \d2(-3, 4)
    \class(-4, 8)
    \class(-2, 8)
    \class(0, 8)
    \class(2, 8)
    \class(4, 8)
    \d2(-3, 6)
    \d2(-1, 6)
    \d2(1, 6)
    \d2(3, 6)
    \d2(5, 6)
    \end{sseqpage}
    \caption{The Adams graded $E_2$ page of the HFPSS computing the homotopy groups $\pi_*\big(k^{tC_{p^n}}\big)$ for $n \geq 2$.}
    \label{fig:E2ktCpn}
\end{figure}
    
    Since we understand the ring structure of $\pi_*(k^{tC_2}) \cong k[t^{\pm1}]$, we can import all differentials from the HFPSS computing $\pi_{t - s} (k^{hC_{2^n}})$ by using multiplicativity and the Leibniz rule. For example, we determine that $d_2(e)e^{-1} = d_2(e^{-1})e$, hence $d_2(e^{-1}) = e^{-2}x^2$.
    
    For degree reasons, this spectral sequence also collapses at the $E_3 = E_\infty$ page (Figure \ref{fig:E2ktCpn}), and we can then read off the homotopy groups of $\pi_{-*}(k^{tC_{2^n}}) \cong \wh{H}^*(C_{2^n};k)$:
$$\wh{H}^*(C_{2^n};k) = k[x_1, e_2^{\pm1}]/(x_1^2)\,\text{.}$$
    
    We now use this information to compute the Tate spectral sequence (Figure \ref{fig:tcp-E2tatess})
\[E_2^{s,t} \cong \widehat{H}^{-s}\big(C_{2^{n-1}}; \pi_t(k^{tC_2})\big) \Rightarrow \pi_*\big((k^{hC_2})^{C_{2^{n-1}}}\big)\,\text{.}\]

As the $C_{2^{n-1}}$-HFPSS computing $\pi_*(k^{hC_{2^n}})$ maps into the $C_{2^{n-1}}$-Tate spectral sequence computing $\pi_*\big((k^{hC_2})^{C_{2^{n-1}}}\big)$, we can then import the $d_2$ differentials.  These differentials also spawn the other $d_2$ differentials in negative Tate cohomology via the ring structure of $\widehat{H}^*\big(C_{2^{n-1}};k\big)$ and the Leibniz rule. As a result, we see that the Tate construction is contractible.
    
\begin{figure}

    \centering
\DeclareSseqGroup\polynomial {} {
\class(0,0)
\DoUntilOutOfBounds {
\class(\lastx-1,\lasty+1)
}
}
\DeclareSseqGroup\tatepolynomial {} {
\class(0,0)
\DoUntilOutOfBounds {
\class(\lastx+1,\lasty-1)
}
}

\begin{sseqpage}[ 
class placement transform = { rotate = 90 }, 
Adams grading,
yscale =0.8,
xscale =0.8,
x tick step = 2, 
y tick step = 2, 
x range = {-2}{6},
y range = {-4}{3},
grid = chess]

\polynomial[](-2,0)
\polynomial[](-1,0)
\polynomial[](0,0)
\polynomial[](1,0)
\polynomial[](2,0)
\polynomial[](3,0)
\polynomial[](4,0)
\polynomial[](5,0)
\polynomial[](6,0)
\polynomial[](7,0)
\polynomial[](8,0)
\polynomial[](9,0)

\tatepolynomial[](2,-1)
\tatepolynomial[](3,-1)
\tatepolynomial[](4,-1)
\tatepolynomial[](5,-1)
\tatepolynomial[](6,-1)
\tatepolynomial[](1,-1)
\tatepolynomial[](0,-1)
\tatepolynomial[](-1,-1)
\tatepolynomial[](-2,-1)
\tatepolynomial[](-3,-1)
\tatepolynomial[](-4,-1)
\tatepolynomial[](-5,-1)


\d2(-2, -3)
\d2(-1, -4)

\d2(-2, -1)
\d2(-1, -2)
\d2(0, -3)
\d2(1, -4)

\d2(-2, 1)
\d2(-1, 0)
\d2(0, -1)
\d2(1, -2)
\d2(2, -3)
\d2(3, -4)

\d2(0, 1)
\d2(1, 0)
\d2(2, -1)
\d2(3, -2)
\d2(4, -3)
\d2(5, -4)

\d2(2, 1)
\d2(3, 0)
\d2(4, -1)
\d2(5, -2)
\d2(6, -3)
\d2(7, -4)

\d2(4, 1)
\d2(5, 0)
\d2(6, -1)
\d2(7, -2)

\d2(6, 1)
\d2(7, 0)

\end{sseqpage}
    \caption{\label{fig:tcp-E2tatess}The Adams graded $E_2$ page of the Tate spectral sequence computing the homotopy groups $\pi_*\big((k^{tC_p})^{tC_{p^{n-1}}}\big)$ for $n \geq 2$.}
\end{figure}    
    
    
    
    
    
    
    
    If $p$ is odd, then the multiplicative structure of the Hochschild--Serre spectral sequence changes. One has
    \[E_2 \cong H^*\big(C_{p^{n-1}};k\big) \otimes H^*(C_p;k) \cong k[x_1,x_2] / (x_1^2) \otimes k[e_1,e_2] / (e_1^2)\,\text{,}\]
    where $e_1$ and $x_1$ are in degree~$1$, and $e_2$ and $x_2$ are in degree~$2$. The $E_2$-page has been illustrated in \cref{E2lhsCp}. One has $d_2(e_1) = x_2$, while $d_2(e_2) = 0$. The resulting $E_3$-page is identical to the case $p = 2$, and once again the spectral sequence collapses (\cref{E3lhsC2}).  We can then read off the homotopy groups of $\pi_{-*}(k^{tC_{p^n}}) \cong \wh{H}^*(C_{p^n};k)$:
$$\wh{H}^*(C_{p^n};k) = k[x_1, e_2^{\pm1}]/(x_1^2)\,\text{.}$$
    
    We once more compute the Tate spectral sequence (Figure \ref{fig:tcp-E2tatess}) in the same way.  We can import $d_2$ differentials from the $C_{p^{n-1}}$-HFPSS computing $\pi_*(k^{hC_{2^n}})$, and our understanding of the ring structure $\widehat{H}^*\big(C_{p^{n-1}};k\big)$ allows us to use multiplicativity to compute the other $d_2$ differentials. Therefore, the Tate construction is again contractible.
    
    \begin{figure}
        \centering
        \begin{sseqpage}[
        Adams grading,
        yscale =0.8,
        xscale =0.8,
        x tick step = 2, 
        x range = {-6}{2},
        y range = {0}{5},
        x label = {$t - s$},
        y label = {$s$},
        grid = chess, 
        classes = { minimum width = 0.2cm, minimum height = 0.2cm },
        run off = .-.]
        \class(0, 0)
        \class["e_1" {right, xshift = -0.2cm}](-1, 0)
        \class["x_1" {right, xshift = -0.2cm}](-1, 1)
        \class["e_2" {right, xshift = -0.2cm}](-2, 0)
        \class(-2, 1)
        \class["x_2" {right, xshift = -0.2cm}](-2, 2)
        \class(-3, 0)
        \class(-3, 1)
        \class(-3, 2)
        \class(-3, 3)
        \class(-4, 0)
        \class(-4, 1)
        \class(-4, 2)
        \class(-4, 3)
        \class(-4, 4)
        \class(-5, 0)
        \class(-5, 1)
        \class(-5, 2)
        \class(-5, 3)
        \class(-5, 4)
        \class(-5, 5)
        \class(-6, 0)
        \class(-6, 1)
        \class(-6, 2)
        \class(-6, 3)
        \class(-6, 4)
        \class(-6, 5)
        \d2(-1, 0)
        \d2(-3, 0)
        \d2(-5, 0)
        \d2(-2, 1)
        \d2(-4, 1)
        \class(-7, 3)
        \d2(-6, 1)
        \d2(-3, 2)
        \d2(-5, 2)
        \d2(-4, 3)
        \class(-7, 5)
        \d2(-6, 3)
        \class(-6, 6)
        \d2(-5, 4)
        \class(-7, 7)
        \d2(-6, 5)
        \end{sseqpage}
            \caption{$E_2$-page of the Hochschild--Serre spectral sequence for the extension $C_p \to C_{p^n} \to C_{p^{n-1}}$, where $p$ is now odd. Compare with \cref{E2lhsC2}.}
        \label{E2lhsCp}
    \end{figure}
    
\end{proof}



\section{For $Q_8$}

\begin{thm}
\label{thm:ktq8faithful}
	The natural ring map $k^{tQ_8} \to k^{tC_2}$ is a \textbf{faithful} $C_2^2$-Galois extension of $\mathbb{E}_\infty$-rings.
\end{thm}

We treat the $Q_8$ case separately from the generalized quaternion case $Q_{2^n}$ because the group cohomology and Tate cohomology rings differ between these two cases, as do the resulting differentials. 

\begin{proof}
    Our method is the same as in the cyclic $p$-group case: we first study the Hochschild--Serre spectral sequence associated to the extension $C_2 \to Q_{8} \to C_2^2$, and then leverage multiplicativity twice to compute the Tate spectral sequence
	\[ E_2^{st} \cong \wh{H}^{s}\big(C_2^2;\pi_t k^{tC_2}\big) \Ra \pi_{t - s} (k^{tC_2})^{tC_2^2}\,\text{.}\]

    \begin{figure}
    \centering
    \begin{sseqpage}[
    Adams grading,
    yscale =0.8,
xscale =0.8,
    x tick step = 2, 
    x range = {-6}{2},
    y range = {0}{5},
    x label = {$t - s$},
    y label = {$s$},
    grid = chess, 
    classes = { minimum width = 0.2cm, minimum height = 0.2cm },
    run off = .-.]
    
    \class(-6, 0)
    \class(-6, 1)
    \class(-6, 1)
    \class(-6, 2)
    \class(-6, 2)
    \class(-6, 2)
    \class(-6, 3)
    \class(-6, 3)
    \class(-6, 3)
    \class(-6, 3)
    \class(-6, 4)
    \class(-6, 4)
    \class(-6, 4)
    \class(-6, 4)
    \class(-6, 4)
    \class(-6, 5)
    \class(-6, 5)
    \class(-6, 5)
    \class(-6, 5)
    \class(-6, 5)
    \class(-6, 5)
    \class(-5, 0)
    \class(-5, 1)
    \class(-5, 1)
    \class(-5, 2)
    \class(-5, 2)
    \class(-5, 2)
    \class(-5, 3)
    \class(-5, 3)
    \class(-5, 3)
    \class(-5, 3)
    \class(-5, 4)
    \class(-5, 4)
    \class(-5, 4)
    \class(-5, 4)
    \class(-5, 4)
    \class(-5, 5)
    \class(-5, 5)
    \class(-5, 5)
    \class(-5, 5)
    \class(-5, 5)
    \class(-5, 5)
    \class(-4, 0)
    \class(-4, 1)
    \class(-4, 1)
    \class(-4, 2)
    \class(-4, 2)
    \class(-4, 2)
    \class(-4, 3)
    \class(-4, 3)
    \class(-4, 3)
    \class(-4, 3)
    \class(-4, 4)
    \class(-4, 4)
    \class(-4, 4)
    \class(-4, 4)
    \class(-4, 4)
    \class(-3, 0)
    \class(-3, 1)
    \class(-3, 1)
    \class(-3, 2)
    \class(-3, 2)
    \class(-3, 2)
    \class(-3, 3)
    \class(-3, 3)
    \class(-3, 3)
    \class(-3, 3)
    \class(-2, 0)
    \class(-2, 1)
    \class(-2, 1)
    \class(-2, 2)
    \class(-2, 2)
    \class(-2, 2)
    \class["e" {right, xshift = -0.2cm, yshift = -0.3cm}](-1, 0)
    \class["x{,} y" {right, xshift = -0.2cm, yshift = -0.3cm}](-1, 1)
    \class(-1, 1)
    \class(-0, 0)
    \d2(-1, 0, , 2)
    \d2(-3, 0, , 2)
    \d2(-5, 0, , 2)
    \d2(-2, 1) \d2(-2, 1, 2, 2)
    \d2(-4, 1) \d2(-4, 1, 2, 2)
    \class(-7, 3) \class(-7, 3) \class(-7, 3) \class(-7, 3)
    \d2(-6, 1) \d2(-6, 1, 2, 2)
    
    \end{sseqpage}
        \caption{$E_2$-page of the Hochschild--Serre spectral sequence, or equivalently, the $(C_2)^2$-HFPSS, associated to the extension $C_2 \to Q_8 \to C_2 \times C_2$, To prevent cluttering, we have only illustrated the nonzero differentials for small~$s$. Each circle represents a $k$-summand.}
        \label{fig:hq-E2hfpss}
    \end{figure}
	Since $C_2$ is central in $Q_8$, the Hochschild--Serre spectral sequence, regraded to match with the grading conventions of the HFPSS, has $E_2$-page of the form
	\[E_2^{s,t} \cong H^{s}((C_2)^2; k) \otimes \pi_t(k^{hC_2})\cong k[x, y] \otimes k[e]\,\text{.}\]
	%I've changed the generators to x, y, e because I used these symbols a ton of times in calculating the unstable differential
	We claim that there are $k$-linear differentials 
	\[d_2(e) = x^2 + xy + y^2 \ \qquad \textnormal{and} \ \qquad d_3(e^2) = x^2 y + xy^2\,\text{.}\]
	As this spectral sequence is multiplicative, we obtain all the other differentials from the Leibniz rule. Note that $d_2(x) = d_2(y) = 0$ for degree reasons.
	
	To see why this is true, recall that by the Kudo transgression theorem, we have that $d_3(e^2) = d_3\big(\textnormal{Sq}^1(e)\big) = \textnormal{Sq}^1 \big(d_2(e)\big)$. Assuming we have proved that $d_2(e) = x^2 + xy + y^2$, we thus obtain that $d_3(e^2) = x^2 y + x y^2$ by computing $\textnormal{Sq}^1(x^2 + xy + y^2)$. Hence it suffices to understand the $d_2$ differential.  We can do so by restricting to appropriate subgroups of $Q_8$, which yields three morphisms of extensions
	\[ \begin{tikzcd}[column sep = huge, row sep = huge]
		1 \ar[r] & C_2 \ar[r] \ar[d] & C_4 \ar[r] \ar[d] & C_2 \ar[d] \ar[r] & 1 \\
		1 \ar[r] & C_2 \ar[r] & Q_8 \ar[r] & C_2 \times C_2 \ar[r] & 1 \end{tikzcd}\]
    all of which induce comparison maps of Hochschild--Serrre spectral sequences for $Q_8$ and for $C_4$. The spectral sequence for $C_4$ had been analysed in the case of $p$-groups (cf. \cref{E2lhsC2}). The $E_3$-page and $E_4$-page have been illustrated in \cref{E3lhsQ8} and \cref{fig:hq-E4hfpss}, respectively.
    
\begin{figure}
\centering
\begin{sseqpage}[
Adams grading,
yscale =0.8,
xscale =0.8,
x tick step = 2, 
x range = {-7}{1},
y range = {0}{6},
x label = {$t - s$},
y label = {$s$},
grid = chess, 
classes = { minimum width = 0.2cm, minimum height = 0.2cm },
run off = .-.]

\class(-6, 0)
\class(-4, 0)
\class(-5, 1)
\class(-5, 1)
\class(-6, 2)
\class(-6, 2)
\class["e^2" {right, xshift = -0.2cm}](-2, 0)
\class(-3, 1)
\class(-3, 1)
\class(-4, 2)
\class(-4, 2)
\class(-5, 3)
\class(-5, 3)
\class(-6, 4)
\class(-6, 4)
\class(0, 0)
\class(-1, 1)
\class(-1, 1)
\class(-2, 2)
\class(-2, 2)
\class(-3, 3)
\class(-3, 3)
\class(-4, 4)
\class(-4, 4)
\class(-5, 5)
\class(-5, 5)
\class(-6, 6)
\class(-6, 6)
\d3(-2, 0)
\d3(-3, 1) \d3(-3, 1, 2, 2)
\d3(-4, 2) \d3(-4, 2, 2, 2)
\d3(-5, 3) \d3(-5, 3, 2, 2)
\class(-7, 7) \class(-7, 7)
\d3(-6, 4) \d3(-6, 4, 2, 2)
\class(-7, 3) \class(-7, 3)
\d3(-6, 0)
\class(-7, 1)
\class(-7, 1)
\class(-7, 5) 
\class(-7, 5)
\class(-8, 4) \class(-8, 4)
\d3(-7, 1) \d3(-7, 1, 2, 2)
\class(-8, 8) \class(-8, 8)
\d3(-7, 5) \d3(-7, 5, 2, 2)

\end{sseqpage}
    \caption{$E_3$-page of the Hochschild--Serre spectral sequence for $C_2 \to Q_8 \to C_2 \times C_2$. \red{Why are these spectral sequences so off-center?}}
\label{E3lhsQ8}
\end{figure}

\begin{figure}
    \centering
\DeclareSseqGroup\polynomial {} {
\class(0,0)
\DoUntilOutOfBounds {
\class(\lastx-1,\lasty+1)
}
}

\begin{sseqpage}[
Adams grading,
yscale =0.8,
xscale =0.8,
x tick step = 2, 
x range = {-7}{2},
y range = {0}{4},
grid = chess,
classes = { minimum width = 0.2cm, minimum height = 0.2cm },
run off = .-.]

\class(0,0)
\class(-1,1)
\class(-1,1)
\class(-2,2)
\class(-2,2)
\class(-3,3)

\class(-4,0)
\class(-5,1)
\class(-5,1)
\class(-6,2)
\class(-6,2)
\class(-7,3)

\end{sseqpage}
    \caption{\label{fig:hq-E4hfpss} $E_4$-page of the HFPSS computing $\pi_*(k^{hQ_8})$. There are no remaining differentials, and the spectral sequence collapses.}
\end{figure}

We therefore obtain the $E_4 = E_\infty$ page of the spectral sequence (Figure \ref{fig:hq-E4hfpss}), and we can then read off the homotopy groups of $\pi_{-*}(k^{hQ_8}) \cong H^*(Q_8;k)$: 
$$H^*(Q_8;k) = k[x_1, x_2, e_4]/(x_1^2 + x_1x_2 + x_2^2, x_1^2x_2 + x_1x_2^2)\,\text{.}$$
	
Alternatively, recall that we can compute the $E_\infty$ page by realizing $\pi_{-*}(k^{hQ_8}) \cong H^{*}(Q_8;k)$ as group cohomology.  We can calculate the latter algebraically through explicit resolutions of $k$ as a $kQ_8$ module, for instance.

We can now again compute $\pi_{t - s} (k^{tQ_8})$ via the HFPSS.  Again, since we understand the ring structure of $\pi_*(k^{tC_2}) \cong k[t^{\pm1}]$, we can import all differentials from the HFPSS computing $\pi_{t - s} (k^{hQ_8})$ by using multiplicativity and the Leibniz rule. Recall that the $E_2$ page (Figure \ref{fig:tq-E2hfpss}) is given by
$$E_2^{s,t} \cong H^{-s}\big((C_2)^2; \pi_t(k^{tC_2})\big) \Rightarrow \pi_*\big((k^{tQ_8}\big)\,\text{.}$$

For degree reasons, this spectral sequence also collapses at the $E_4 = E_\infty$ page (Figure \ref{fig:tq-E4hfpss}), and we can then read off the homotopy groups of $\pi_{-*}(k^{tQ_8}) \cong \wh{H}^*(Q_8;k)$:
$$\wh{H}^*(Q_8;k) = k[x_1, x_2, e_4^{\pm1}]/(x_1^2 + x_1x_2 + x_2^2, x_1^2x_2 + x_1x_2^2)\,\text{.}$$

We now use this information to compute the Tate spectral sequence (Figure \ref{fig:tq-E2tatess})
\[E_2^{s,t} \cong \widehat{H}^{-s}\big((C_2)^2; \pi_*(k^{hC_2})\big) \Rightarrow \pi_*\big((k^{hC_2})^{t(C_2)^2}\big)\,\text{.}\]
Recall that since the cohomology of $(C_2)^2$ is Cohen--Macaulay, we can explicitly describe the multiplicative structure of $\widehat{H}^*\big((C_2)^2;k\big)$ via the {\v C}ech cohomology spectral sequence (see \cref{thm:tate-mult}).  

In positive degrees, $\widehat{H}^*\big((C_2)^2;k\big)$ has the multiplicative structure of $H^*\big((C_2)^2;k\big)$; in negative degrees, there is a polynomial algebra $k[x_1^{-1},x_2^{-1}]$ generated by a class $\alpha$ in degree $-1$.  That is, any element in negative degree Tate cohomology is of the form $\alpha x_1^{-a}x_2^{-b}$.  Hence, the multiplication in negative degrees is determined by the relations $$\alpha^2 = \alpha \cdot x_1 = \alpha \cdot x_2 = 0\,\text{.}$$

As the $(C_2)^2$-HFPSS computing $\pi_*(k^{hQ_8})$ maps into the $(C_2)^2$-Tate spectral sequence computing $\pi_*\big((k^{hC_2})^{t(C_2)^2}\big)$, we can then import the $d_2$ and $d_3$ differentials.  These differentials also spawn the other differentials in negative Tate cohomology through the multiplicative structure. In particular, the new noteworthy differentials come from $$t^{-1} \alpha x_1^{-a}x_2^{-b} \text{ with } a, b \geq 0, a+b \geq 2\text{,}$$
and
$$t^{-3} \alpha x_1^{-a}x_2^{-b} \text{ with } a \geq 2, b \geq 1,  \text{ or } a \geq 1, b \geq 2\text{.}$$
By the Leibniz rule, we have that 
\begin{align*}
    d_2(t^{-1} \alpha x_1^{-a}x_2^{-b}) &= d_2(t^{-1}) \cdot \alpha x_1^{-a}x_2^{-b} \\
    &= \alpha (x_1^{2-a}x_2^{-b} + x_1^{1-a}x_2^{1-b} + x_1^{-a}x_2^{2-b})\,\text{;}
\end{align*}
similarly,
\begin{align*}
    d_3(t^{-3} \alpha x_1^{-a}x_2^{-b}) &= d_3(t^{-3}) \cdot \alpha x_1^{-a}x_2^{-b} \\
    &= t^{-1} \alpha (x_1^{2-a}x_2^{1-b} + x_1^{1-a}x_2^{2-b})\,\text{.}
\end{align*}
Therefore, given these restrictions on $a$ and $b$, we obtain non-zero $d_2$ and $d_3$ differentials in the Tate spectral sequence. It remains to show that there are non-trivial $d_4$ differentials (Figure \ref{fig:tq-E4tatess}).

We argue first that $\pi_0((k^{hC_2})^{tC_2^2})$ is trivial.   We do so by considering the cofiber sequence 
$$(k^{hC_2})_{hC_2^2} \xrightarrow{\textnormal{Norm}_{C_2^2}} (k^{hC_2})^{hC_2^2} \to (k^{hC_2})^{tC_2^2}$$

We have shown that the middle term $(k^{hC_2})^{hC_2^2} \simeq k^{hQ_8}$, hence $\pi_0(k^{hQ_8}) \cong k$.  Moreover, computing the homotopy orbit spectral sequence in low degrees shows that for degree reasons, $\pi_{-1}((k^{hC_2})_{hC_2^2}) \cong 0$, and $\pi_{0}((k^{hC_2})_{hC_2^2}) \cong k$.  Furthermore, we know that $\pi_0$ is the norm map, which is an isomorphism.  Hence $\pi_0((k^{hC_2})^{tC_2^2})$ is trivial \blue{Check with Andrew/Jesper}.

Therefore, for degree reasons, the potential $d_4$ differential from the Adams-graded $(1,-4)$ spot is forced to be an isomorphism.  By multiplicativity, this forces the rest of the $d_4$ differentials to be isomorphisms as well.  Hence $(k^{hC_2})^{tC_2^2}$ is contractible, so we have shown that $k^{hQ_8} \to k^{hC_2}$ is a faithful Galois extension.

Once more by multiplicativity, we further obtain that $(k^{tC_2})^{tC_2^2}$ is contractible, hence $k^{tQ_8} \to k^{tC_2}$ is a faithful Galois extension as well.

In fact, this also shows that we have equivalence $(k^{hC_2})_{hC_2^2} \simeq (k^{hC_2})^{hC_2^2}$ and $(k^{tC_2})_{hC_2^2} \simeq (k^{tC_2})^{hC_2^2}$.

% \blue{TEST. Is the following argument too strong?}

% \label{Proof 1}

% We have the following square of cofiber sequences.

% \begin{tikzcd}
% (k^{tC_2})_{hC_2^2} \arrow[r]           & (k^{tC_2})^{hC_2^2} \arrow[r]           & (k^{tC_2})^{tC_2^2}           \\
% (k^{hC_2})_{hC_2^2} \arrow[r] \arrow[u] & (k^{hC_2})^{hC_2^2} \arrow[r] \arrow[u] & (k^{hC_2})^{tC_2^2} \arrow[u] \\
% (k_{hC_2})_{hC_2^2} \arrow[r] \arrow[u] & (k_{hC_2})^{hC_2^2} \arrow[r] \arrow[u] & (k_{hC_2})^{tC_2^2} \arrow[u]
% \end{tikzcd}

% We can identify the relevant terms as follows.  We obtain the bottom middle term as the fiber of $k^{hQ_8} \to k^{tQ_8}$.  This forces the bottom right term to be 0.  I think it should also force the middle left term to be $k^{hQ_8}$, which forces the middle right to be 0 as desired?

% \begin{tikzcd}
% (k^{tC_2})_{hC_2^2} \arrow[r]           & \red{k^{tQ_8}} \arrow[r]           & (k^{tC_2})^{tC_2^2}           \\
% (k^{hC_2})_{hC_2^2} \arrow[r] \arrow[u] & \red{k^{hQ_8}} \arrow[r] \arrow[u] & (k^{hC_2})^{tC_2^2} \arrow[u] \\
% \blue{k_{hQ_8}} \arrow[r] \arrow[u]     & \red{k_{hQ_8}} \arrow[r] \arrow[u] & \blue{0} \arrow[u]           
% \end{tikzcd}

% If this doesn't work, then we should still be able to argue from the middle row cofiber sequence $(k^{hC_2})_{hC_2^2} \to (k^{hC_2})^{hC_2^2} \to  (k^{hC_2})^{tC_2^2}$ at $\pi_0$ where the first two terms should be $k$ and the norm map should be an isomorphism...

\end{proof}


\begin{figure}[H]
    \centering
\DeclareSseqGroup\polynomial {} {
\class(0,0)
\DoUntilOutOfBounds {
\class(\lastx-1,\lasty+1)
}
}
\begin{sseqpage}[ 
class placement transform = { rotate = 90 }, 
Adams grading,
yscale =0.8,
xscale =0.8,
x tick step = 2, 
x range = {-2}{6},
y range = {0}{3},
grid = chess]
\polynomial[](0,0)
\polynomial[](-1,1)
\polynomial[](-2,2)
\polynomial[](-3,3)
\polynomial[](-4,4)


\class(-1,0)
\d2
\DoUntilOutOfBounds{
\class(\lastx-1,\lasty+1)
%\d2
}
\polynomial[](-2,1)
\polynomial[](-3,2)
\polynomial[](-4,3)
\polynomial[](-5,4)
\polynomial[](-2,0)

\polynomial[](1,0)
\polynomial[](0,1)
\polynomial[](-1,2)
\polynomial[](-2,3)
\polynomial[](-3,4)

\polynomial[](2,0)
\polynomial[](1,1)
\polynomial[](0,2)
\polynomial[](-1,3)
\polynomial[](-2,4)

\polynomial[](3,0)
\polynomial[](2,1)
\polynomial[](1,2)
\polynomial[](0,3)
\polynomial[](-1,4)
\polynomial[](4,0)
\polynomial[](3,1)
\polynomial[](2,2)
\polynomial[](1,3)
\polynomial[](0,4)
\polynomial[](5,0)
\polynomial[](4,1)
\polynomial[](3,2)
\polynomial[](2,3)
\polynomial[](1,4)
\polynomial[](6,0)
\polynomial[](5,1)
\polynomial[](4,2)
\polynomial[](3,3)
\polynomial[](2,4)
\polynomial[](7,0)
\polynomial[](6,1)
\polynomial[](5,2)
\polynomial[](4,3)
\polynomial[](3,4)
\polynomial[](8,0)
\polynomial[](7,1)
\polynomial[](6,2)
\polynomial[](5,3)
\polynomial[](4,4)
\polynomial[](9,0)
\polynomial[](8,1)
\polynomial[](7,2)
\polynomial[](6,3)
\polynomial[](5,4)



% \d2(-5,0)
% \d2(-3,0)
%\d2(-1,0)
\d2(1,0)
\d2(3,0)
\d2(5,0)

\d3(-2,0)
\d3(2,0)
\d3(6,0)

\end{sseqpage}

    \caption{\label{fig:tq-E2hfpss}The Adams graded $E_2$ page of the $(Q_{2^n}/C_2)$-HFPSS computing $\pi_*(k^{tQ_{2^n}})$ for $n \geq 3$. $\circ = k$. Not all differentials are drawn.}
\end{figure}

\begin{figure}[H]
    \centering
\DeclareSseqGroup\polynomial {} {
\class(0,0)
\DoUntilOutOfBounds {
\class(\lastx-1,\lasty+1)
}
}

\begin{sseqpage}[ 
class placement transform = { rotate = 90 }, 
Adams grading,
yscale =0.8,
xscale =0.8,
x tick step = 2, 
x range = {-5}{4},
y range = {0}{4},
grid = chess]

\class(0,0)
\class(-1,1)
\class(-1,1)
\class(-2,2)
\class(-2,2)
\class(-3,3)

\class(-4,0)
\class(-5,1)
\class(-5,1)
\class(-6,2)
\class(-6,2)
\class(-7,3)

\class(4,0)
\class(3,1)
\class(3,1)
\class(2,2)
\class(2,2)
\class(1,3)

\end{sseqpage}
    \caption{\label{fig:tq-E4hfpss}The Adams graded $E_4 = E_\infty$ page of the $(Q_{2^n}/C_2)$-HFPSS computing $\pi_*(k^{tQ_{2^n}})$ for $n \geq 3$. $\circ = k$.}
\end{figure}


\begin{figure}[H]

    \centering
\DeclareSseqGroup\polynomial {} {
\class(0,0)
\DoUntilOutOfBounds {
\class(\lastx-1,\lasty+1)
}
}
\DeclareSseqGroup\tatepolynomial {} {
\class(0,0)
\DoUntilOutOfBounds {
\class(\lastx+1,\lasty-1)
}
}

\begin{sseqpage}[ 
class placement transform = { rotate = 90 }, 
Adams grading,
yscale =0.8,
xscale =0.8,
x tick step = 2, 
y tick step = 2, 
x range = {-2}{6},
y range = {-4}{3},
grid = chess]
\polynomial[](0,0)
\polynomial[](-1,1)
\polynomial[](-2,2)
\polynomial[](-3,3)
\polynomial[](-4,4)


\class(-1,0)
\d2
\DoUntilOutOfBounds{
\class(\lastx-1,\lasty+1)
%\d2
}
\polynomial[](-2,1)
\polynomial[](-3,2)
\polynomial[](-4,3)
\polynomial[](-5,4)
\polynomial[](-2,0)

\polynomial[](1,0)
\polynomial[](0,1)
\polynomial[](-1,2)
\polynomial[](-2,3)
\polynomial[](-3,4)
\polynomial[](2,0)
\polynomial[](1,1)
\polynomial[](0,2)
\polynomial[](-1,3)
\polynomial[](-2,4)
\polynomial[](3,0)
\polynomial[](2,1)
\polynomial[](1,2)
\polynomial[](0,3)
\polynomial[](-1,4)
\polynomial[](4,0)
\polynomial[](3,1)
\polynomial[](2,2)
\polynomial[](1,3)
\polynomial[](0,4)
\polynomial[](5,0)
\polynomial[](4,1)
\polynomial[](3,2)
\polynomial[](2,3)
\polynomial[](1,4)
\polynomial[](6,0)
\polynomial[](5,1)
\polynomial[](4,2)
\polynomial[](3,3)
\polynomial[](2,4)
\polynomial[](7,0)
\polynomial[](6,1)
\polynomial[](5,2)
\polynomial[](4,3)
\polynomial[](3,4)
\polynomial[](8,0)
\polynomial[](7,1)
\polynomial[](6,2)
\polynomial[](5,3)
\polynomial[](4,4)
\polynomial[](9,0)
\polynomial[](8,1)
\polynomial[](7,2)
\polynomial[](6,3)
\polynomial[](5,4)

\tatepolynomial[](2,-1)
\tatepolynomial[](3,-2)
\tatepolynomial[](4,-3)
\tatepolynomial[](5,-4)
\tatepolynomial[](6,-5)
\tatepolynomial[](3,-1)
\tatepolynomial[](4,-2)
\tatepolynomial[](5,-3)
\tatepolynomial[](6,-4)
\tatepolynomial[](7,-5)
\tatepolynomial[](4,-1)
\tatepolynomial[](5,-2)
\tatepolynomial[](6,-3)
\tatepolynomial[](7,-4)
\tatepolynomial[](8,-5)
\tatepolynomial[](5,-1)
\tatepolynomial[](6,-2)
\tatepolynomial[](7,-3)
\tatepolynomial[](8,-4)
\tatepolynomial[](9,-5)
\tatepolynomial[](6,-1)
\tatepolynomial[](7,-2)
\tatepolynomial[](8,-3)
\tatepolynomial[](9,-4)
\tatepolynomial[](10,-5)
\tatepolynomial[](1,-1)
\tatepolynomial[](2,-2)
\tatepolynomial[](3,-3)
\tatepolynomial[](4,-4)
\tatepolynomial[](5,-5)
\tatepolynomial[](0,-1)
\tatepolynomial[](1,-2)
\tatepolynomial[](2,-3)
\tatepolynomial[](3,-4)
\tatepolynomial[](4,-5)
\tatepolynomial[](-1,-1)
\tatepolynomial[](0,-2)
\tatepolynomial[](1,-3)
\tatepolynomial[](2,-4)
\tatepolynomial[](3,-5)
\tatepolynomial[](-2,-1)
\tatepolynomial[](-1,-2)
\tatepolynomial[](0,-3)
\tatepolynomial[](1,-4)
\tatepolynomial[](2,-5)
\tatepolynomial[](-3,-1)
\tatepolynomial[](-2,-2)
\tatepolynomial[](-1,-3)
\tatepolynomial[](0,-4)
\tatepolynomial[](1,-5)
\tatepolynomial[](-4,-1)
\tatepolynomial[](-3,-2)
\tatepolynomial[](-2,-3)
\tatepolynomial[](-1,-4)
\tatepolynomial[](0,-5)
\tatepolynomial[](-5,-1)
\tatepolynomial[](-4,-2)
\tatepolynomial[](-3,-3)
\tatepolynomial[](-2,-4)


% \d2(-5,0)
% \d2(-3,0)
%\d2(-1,0)
\d2(1,0)
\d2(3,0)
\d2(5,0)

\d2(6,-3)
\d2(4,-3)
\d2(2,-3)
\d2(0,-3)
\d2(-2,-3)
% \d2(-4,-3)
% \d2(-6,-3)

\d3(-2,0)
\d3(2,0)
\d3(6,0)

\d3(5,-4)
\d3(1,-4)
%\d3(-3,-4)
%\d3(-7,-4)


\end{sseqpage}
    \caption{\label{fig:tq-E2tatess}The Adams graded $E_2$ page of the Tate spectral sequence computing the homotopy groups $\pi_*\big((k^{tC_2})^{tQ_{2^n}/C_2}\big)$ for $n \geq 3$.  Not all differentials are drawn.}
\end{figure}

\begin{figure}[H]
    \centering
\DeclareSseqGroup\polynomial {} {
\class(0,0)
\DoUntilOutOfBounds {
\class(\lastx-1,\lasty+1)
}
}
\DeclareSseqGroup\tatepolynomial {} {
\class(0,0)
\DoUntilOutOfBounds {
\class(\lastx+1,\lasty-1)
}
}

\begin{sseqpage}[ 
Adams grading,
yscale =0.8,
xscale =0.8,
x tick step = 2, 
y tick step = 2, 
x range = {-2}{6},
y range = {-5}{4},
grid = chess]



\class(0,0)
\class(-1,1)
\class(-1,1)
\class(-2,2)
\class(-2,2)
\class(-3,3)

\class(4,0)
\class(3,1)
\class(3,1)
\class(2,2)
\class(2,2)
\class(1,3)

\class(8,0)
\class(7,1)
\class(7,1)
\class(6,2)
\class(6,2)
\class(5,3)

\class(-2,-1)
\class(-1,-2)
\class(-1,-2)
\class(0,-3)
\class(0,-3)
\class(1,-4)

\class(2,-1)
\class(3,-2)
\class(3,-2)
\class(4,-3)
\class(4,-3)
\class(5,-4)

\class(6,-1)
\class(7,-2)
\class(7,-2)
\class(8,-3)
\class(8,-3)
\class(9,-4)

\d4(1,-4)
\d4(0,-3)
\d4(0,-3,2,2)
\d4(-1,-2)\d4(-1,-2,2,2)
\d4(-2,-1)

\d4(5,-4)
\d4(4,-3)\d4(4,-3,2,2)
\d4(3,-2)\d4(3,-2,2,2)
\d4(2,-1)

\d4(6,-1)

\end{sseqpage}
    \caption{\label{fig:tq-E4tatess}The Adams graded $E_4$ page of the Tate spectral sequence computing $\pi_*((k^{tC_2})^{tQ_{2^n}/C_2})$ for $n \geq 3$.}
\end{figure}

\section{For $Q_{2n}$}

\begin{thm}
\label{thm:ktq2nfaithful}
	The natural ring map $k^{tQ_{2^n}} \to k^{tC_2}$ is a \textbf{faithful} $Q_{2^n}/C_2$-Galois extension of $\mathbb{E}_\infty$-rings.
\end{thm}

\begin{proof}
    Our method is the same as in the previous cases - we first study the LHS spectral sequence associated to the fiber sequence $BC_2 \to BQ_{2^n} \to BD_{2^{n-1}}$, and then leverage multiplicativity twice to compute the Tate spectral sequence (Figure \ref{fig:tq-E2tatess})
	\[ E_2^{st} \cong \wh{H}^{s}\big(D_{2^{n-1}};\pi_t k^{tC_2}\big) \Ra \pi_{t - s} (k^{tC_2})^{tD_{2^{n-1}}}\,\text{.}\]
	
	Recall that for $n \geq 4$, $H^*(D_{2^{n-1}};k) \cong k[x_1, x_2, z]/(x_1x_2)$, where $|x_i| = 1$ and $|z| = 2$. Moreover, $\textnormal{Sq}^1(z) = (x_1+x_2)z$.  It is convenient to set $u = x_1 + x_2$ and write
$$H^*(D_{2^{n-1}}; k) \cong k[x_1,u, z]/(ux_1 +x_1^2 = 0)$$

We first recall that since $C_2$ is central in $Q_{2^n}$, the LHS spectral sequence (regraded to match the HFPSS computing $\pi_{t - s} (k^{hQ_8})$) has $E_2$ page (Figure \ref{fig:hq2n-E2hfpss}) of the form
	\[E_2^{s,t} \cong H^{s}(D_{2^{n-1}}; k) \otimes \pi_t(k^{hC_2})\cong k[x_1, x_2, z]/(x_1x_2) \otimes k[t]\,\text{,}\]
	where the $x_i$ are in the Adams-graded (-1,1) spot, $z$ is in the Adams-graded (-2,2) spot and $t$ is in the Adams-graded (-1,0) spot.  We have $k$-linear differentials
	\[d_2(t) = x_1^2 + x_2^2 + z \ \qquad \textnormal{and} \ \qquad d_3(t^2) = uz\,\text{.}\]
	which again spawn all the other differentials from the Leibniz rule.   
	
	We again obtain the $d_3$ differential from the $d_2$ differential via the Kudo transgression theorem, and we can compute the $d_2$ differential.  We do so by again by restricting to appropriate subgroups. 

\begin{figure}
    \centering
\DeclareSseqGroup\polynomial {} {
\class(0,0)
\DoUntilOutOfBounds {
\class(\lastx-1,\lasty+1)
}
}
\begin{sseqpage}[ 
class placement transform = { rotate = 90 }, 
Adams grading,
yscale =0.8,
xscale =0.8,
x tick step = 2, 
x range = {-7}{1},
y range = {0}{3},
grid = chess]
\polynomial[](0,0)
\polynomial[](-1,1)
\polynomial[](-2,2)
\polynomial[](-3,3)
\polynomial[](-4,4)


\class(-1,0)
\d2
\DoUntilOutOfBounds{
\class(\lastx-1,\lasty+1)
%\d2
}
\polynomial[](-2,1)
\polynomial[](-3,2)
\polynomial[](-4,3)
\polynomial[](-5,4)

\polynomial[](-2,0)
\polynomial[](-3,1)
\polynomial[](-4,2)
\polynomial[](-5,3)
\polynomial[](-6,4)

\polynomial[](-3,0)
\polynomial[](-4,1)
\polynomial[](-5,2)
\polynomial[](-6,3)
\polynomial[](-7,4)

\polynomial[](-4,0)
\polynomial[](-5,1)
\polynomial[](-6,2)
\polynomial[](-7,3)
\polynomial[](-8,4)

\polynomial[](-5,0)
\polynomial[](-6,1)
\polynomial[](-7,2)
\polynomial[](-8,3)
\polynomial[](-9,4)

\polynomial[](-6,0)
\polynomial[](-7,1)
\polynomial[](-8,2)
\polynomial[](-9,3)
\polynomial[](-10,4)

\polynomial[](-7,0)

 \d2(-5,0)
 \d2(-3,0)

\d3(-2,0)
\d3(-6,0)

\end{sseqpage}

    \caption{\label{fig:hq2n-E2hfpss}The Adams-graded HFPSS computing $\pi_*(k^{hQ_{2^n}})$. $\circ = k$. Not all differentials are drawn.}
\end{figure}

\begin{figure}
    \centering
\DeclareSseqGroup\polynomial {} {
\class(0,0)
\DoUntilOutOfBounds {
\class(\lastx-1,\lasty+1)
}
}

\begin{sseqpage}[ 
class placement transform = { rotate = 90 }, 
Adams grading,
yscale =0.8,
xscale =0.8,
x tick step = 2, 
x range = {-7}{1},
y range = {0}{4},
grid = chess]

\class(0,0)
\class(-1,1)
\class(-1,1)
\class(-2,2)
\class(-2,2)
\class(-3,3)

\class(-4,0)
\class(-5,1)
\class(-5,1)
\class(-6,2)
\class(-6,2)
\class(-7,3)


\end{sseqpage}
    \caption{\label{fig:hq2n-E4hfpss}The Adams graded $E_4 = E_\infty$ page of the HFPSS computing $\pi_*(k^{hQ_{2^n}})$.}
\end{figure}

We therefore obtain the $E_4 = E_\infty$ page of the spectral sequence (Figure \ref{fig:hq2n-E4hfpss}), and we can then read off the homotopy groups of $\pi_{-*}(k^{hQ_{2^n}}) \cong H^*(Q_{2^n};k)$:
$$H^*(Q_{2^n};k) \cong k[x_1, x_2, e_4]/(x_1^2 + x_1x_2, x_1^3 + x_2^3)\,\text{.}$$

We can now again compute $\pi_{t - s} (k^{tQ_{2^n}})$ via the HFPSS.  Again, since we understand the ring structure of $\pi_*(k^{tC_2}) \cong k[t^{\pm1}]$, we can import all differentials from the HFPSS computing $\pi_{t - s} (k^{hQ_8})$ by using multiplicativity and the Leibniz rule. Recall that the $E_2$ page (Figure \ref{fig:tq-E2hfpss}) is given by
\[E_2^{s,t} \cong H^{s}(D_{2^{n-1}}; k) \otimes \pi_t(k^{hC_2})\cong k[x_1, x_2, z]/(x_1x_2) \otimes k[t^{\pm1}]\,\text{,}\]

For degree reasons, this spectral sequence also collapses at the $E_4 = E_\infty$ page (Figure \ref{fig:tq-E4hfpss}), and we can then read off the homotopy groups of $\pi_{-*}(k^{tQ_{2^n}}) \cong \wh{H}^*(Q_{2^n};k)$:
$$\wh{H}^*(Q_{2^n};k) = k[x_1, x_2, e_4^{\pm1}]/(x_1x_2, x_1^3 + x_2^3)\,\text{.}$$

We now use this information to compute the Tate spectral sequence (Figure \ref{fig:tq-E2tatess})
\[ E_2^{st} \cong \wh{H}^{s}\big(D_{2^{n-1}};\pi_t k^{tC_2}\big) \Ra \pi_{t - s} (k^{tC_2})^{tD_{2^{n-1}}}\,\text{.}\]
Recall that since the cohomology of $D_{2^{n-1}}$ is Cohen--Macaulay, we can explicitly describe the multiplicative structure of $\widehat{H}^*\big(D_{2^{n-1}};k\big)$ via the {\v C}ech cohomology spectral sequence (see \cref{thm:tate-mult}), which allows us to spawn further differentials through the multiplicative structure. In particular, the new noteworthy $d_2$ differentials come from:
$$t^{-1} \alpha u^{-a}z^{-b} \text{ and } t^{-1} \alpha u^{-a}z^{-b}x_1 \text{ with } a, b \geq 0, a+2b \geq 2$$

Noting that $\alpha \cdot u = \alpha \cdot z = 0$, we see that $$d_2(t^{-1} \alpha u^{-a}z^{-b}) = \alpha u^{2-a}z^{-b} + \alpha u^{-a}z^{1-b}$$ 
$$d_2(t^{-1} \alpha u^{-a}z^{-b}x_1) = \alpha u^{2-a}z^{-b}x_1 + \alpha u^{-a}z^{1-b}x_1$$

On the $E_3$ page, note that $t^{-1} \alpha u^{-2} + t^{-1} \alpha z^{-1} = 0$, hence the new noteworthy $d_3$ differentials come from:

$$t^{-3} \alpha u^{-a} \text{ and } t^{-3} \alpha u^{-a}x_1 \text{ with } a \geq 3$$

We see that $$d_3(t^{-3} \alpha u^{-a}) = t^{-1}\alpha u^{3-a} \text{ and } d_3(t^{-3} \alpha u^{-a}x_1) = t^{-1}\alpha u^{3-a}x_1$$ 

Therefore, given these restrictions on $a$ and $b$, we obtain non-zero $d_2$ and $d_3$ differentials in the Tate spectral sequence. It remains to show that there are non-trivial $d_4$ differentials (Figure \ref{fig:tq-E4tatess}), which follows again by the same logic for the $Q_8$ case.

We argue that $\pi_0((k^{hC_2})^{tD_{2^{n-1}}})$ is trivial by considering the cofiber sequence 
$$(k^{hC_2})_{hD_{2^{n-1}}} \xrightarrow{\textnormal{Norm}_{D_{2^{n-1}}}} (k^{hC_2})^{hD_{2^{n-1}}} \to (k^{hC_2})^{tD_{2^{n-1}}}$$

The middle term $(k^{hC_2})^{hD_{2^{n-1}}} \simeq k^{hQ_{2^n}}$, hence $\pi_0(k^{hQ_8}) \cong k$.  Moreover, computing the homotopy orbit spectral sequence in low degrees shows that for degree reasons, $\pi_{-1}((k^{hC_2})_{hD_{2^{n-1}}}) \cong 0$, and $\pi_{0}((k^{hC_2})_{hD_{2^{n-1}}}) \cong k$.  Furthermore, we know that $\pi_0$ is the norm map, which is an isomorphism.   \blue{Check with Andrew/Jesper}. Hence $\pi_0((k^{hC_2})^{tD_{2^{n-1}}})$ is trivial, which forces the $d_4$ differential from the Adams-graded $(1,-4)$ spot to be an isomorphism.  Again this propagates by multiplicativity to show that $(k^{hC_2})^{tD_{2^{n-1}}}$ and $(k^{tC_2})^{tD_{2^{n-1}}}$
are contractible (Figure \ref{fig:tq-E4tatess}), hence we have equivalences $(k^{hC_2})_{hC_2^2} \simeq (k^{hC_2})^{hC_2^2}$ and $(k^{tC_2})_{hC_2^2} \simeq (k^{tC_2})^{hC_2^2}$, as well as faithful Galois extensions.

\end{proof}
	











% \begin{figure}
% \centering
% \begin{tikzpicture}
% 	\matrix(m)[matrix of math nodes, nodes in empty cells, nodes = {minimum width = 10ex, minimum height = 5ex, outer sep = -5pt}, column sep = 1ex, row sep = 1ex]
% 	{              &   &     &     &     & \\
% 	e^{-3} & k^3 & k^2 & k & k & k^2 & k^3 & k^4 & \\
% 	e^{-2} & k^3 & k^2 & k & k & k^2 & k^3 & k^4 & \\
% 	e^{-1} & k^3 & k^2 & k & k & k^2 & k^3 & k^4 & \\
% 	1      & k^3 & k^2 & k & k & k^2 & k^3 & k^4 & \\
% 	e      & k^3 & k^2 & k & k & k^2 & k^3 & k^4 & \\
% 	e^2    & k^3 & k^2 & k & k & k^2 & k^3 & k^4 & \\
% 	e^3    & k^3 & k^2 & k & k & k^2 & k^3 & k^4 & \\
% 	\strut & \ol{x^2}, \ol{xy},\ol{y^2} & \ol{x},\ol{y} & u & 1 & x, y & x^2 , xy , y^2 & x^3 , x^2 y , xy^2 , y^3 & \strut \\};
% 	\draw[-stealth] (m-5-6.north east) -- (m-4-8.south west);
% 	\draw[-stealth] (m-6-5.north east) -- (m-5-7.south west);

% 	\draw[thick] (m-1-1.south east) -- (m-9-1.east);
% 	\draw[thick] (m-9-1.north) -- (m-9-9.north west);
% \end{tikzpicture}
% \caption{$E_2$-page of the Tate spectral sequence computing the homotopy groups of $(k^{tC_2})^{tC_2^2}$. We notice that the right half of the spectral sequence identifies with \cref{E2tateQ8}.}
% \label{E2bigtateQ8}
% \end{figure}

% \begin{figure}
% \centering
% \begin{tikzpicture}
% 	\matrix(m)[matrix of math nodes, nodes in empty cells, nodes = {minimum width = 8ex, minimum height = 5ex, outer sep = -5pt}, column sep = 1ex, row sep = 1ex]
% 	{              &   &     &     &     & \\
% 	e^{-3} & k^2 & k^2 & k^2 & k & 0 & 0 & 0 & 0 & \\
% 	e^{-2} & 0 & 0 & 0 & 0 & k & k^2 & k^2 & k^2 & \\
% 	e^{-1} & k^2 & k^2 & k^2 & k & 0 & 0 & 0 & 0 & \\
% 	1      & 0 & 0 & 0 & 0 & k & k^2 & k^2 & k^2 & \\
% 	e      & k^2 & k^2 & k^2 & k & 0 & 0 & 0 & 0 & \\
% 	e^2    & 0 & 0 & 0 & 0 & k & k^2 & k^2 & k^2 & \\
% 	e^3    & k^2 & k^2 & k^2 & k & 0 & 0 & 0 & 0 & \\
% 	\strut & \ol{x^3},\ol{y^3} & \ol{x^2},\ol{y^2} & \ol{x},\ol{y} & u & 1 & x, y & x^2 , y^2 & x^3 , y^3 & \strut \\};

% 	\draw[-stealth] (m-5-6.north east) -- (m-3-9.south west);
% 	\draw[-stealth] (m-8-2.north east) -- (m-6-5.south west);

% 	\draw[thick] (m-1-1.south east) -- (m-9-1.east);
% 	\draw[thick] (m-9-1.north) -- (m-9-10.north west);
% \end{tikzpicture}
% \caption{$E_3$-page of the Tate spectral sequence computing the homotopy groups of $(k^{tC_2})^{tC_2^2}$. The illustrated differentials are nontrivial, and multiplicativity extends this to further $t$.}
% \label{E3bigtateQ8}
% \end{figure}

